CtRL-Sim: Reactive and Controllable Driving Agents with Offline Reinforcement Learning

Evaluating autonomous vehicle stacks (AVs) in simulation typically involves replaying driving logs from real-world recorded traffic. However, agents replayed from offline data are not reactive and hard to intuitively control. Existing approaches address these challenges by proposing methods that rely on heuristics or generative models of real-world data but these approaches either lack realism or necessitate costly iterative sampling procedures to control the generated behaviours. In this work, we take an alternative approach and propose CtRL-Sim, a method that leverages return-conditioned offline reinforcement learning (RL) to efficiently generate reactive and controllable traffic agents. Specifically, we process real-world driving data through a physics-enhanced Nocturne simulator to generate a diverse offline RL dataset, annotated with various rewards. With this dataset, we train a return-conditioned multi-agent behaviour model that allows for fine-grained manipulation of agent behaviours by modifying the desired returns for the various reward components. This capability enables the generation of a wide range of driving behaviours beyond the scope of the initial dataset, including adversarial behaviours. We show that CtRL-Sim can generate realistic safety-critical scenarios while providing fine-grained control over agent behaviours.

==> sec/3_background.tex <==
\section{Background}
\label{sec:background}

We consider the common offline RL setup where we are given a dataset $\mathcal{D}$ of trajectories $\tau_i=\{\ldots, s_t, a_t, r_t, \ldots\}$, with states $s_t \in \mathcal{S}$, actions $a_t \in \mathcal{A}$ and rewards $r_t$.
These trajectories are generated using a (suboptimal) behaviour policy $\pi_B(a_t|s_t)$ executed in a finite-horizon Markov Decision Process.
The return at timestep $t$ is defined as the cumulative sum of scalar rewards obtained in the trajectory from timestep $t$, $G_t = \sum_{t'=t}^{T} r_{t'}$.
The objective of offline RL is to learn policies that perform as well as or better than the best agent behaviours observed in $\mathcal{D}$.

Prior methods differ in how the policy is modelled during training and how inference is performed; we refer the reader to  Table~\ref{tab:joint_learning_acting} in the Appendix \ref{sec:policy_extract} for a breakdown of the different approaches.
As \ourmodel employs a return-conditioned policy for controllable simulation, we briefly present a class of related methods that learn return-conditioned policies (RCPs)~\citep{chen2021decisiontransformer, lee2022multigamedt, Srivastava2019TrainingAU, kumar2019reward, Emmons2021RvSWI, piche2022probabilistic, Meng2021OfflinePM} for offline RL.
RCPs are concerned with learning the joint distribution of actions and returns, such that action sampling is conditioned on the return distribution.
Most methods will learn the joint distribution by decomposing it and minimizing the following objective:
\begin{equation}
    \mathcal{L}(\theta) = \mathbb{E}_{\{s_t, a_t, G_t\} } \big [ -\log p_\theta(a_t | s_t, G_t) p_\theta(G_t | s_t) \big ].
\end{equation}
Instead of modelling the return distribution, the Decision Transformer~\citep{chen2021decisiontransformer} conditions the learned policy on the maximum observed return, $ G_{\text{max}}$ in the dataset.
That is, at inference time, the actions are sampled from $a_t \sim p_\theta(a_t | s_t, G_{\text{max}})$.
\cite{lee2022multigamedt} instead propose to employ the learned return distribution, combined with exponential tilting, in order to sample high-return actions while remaining close to the empirical distribution.
This effectively amounts to sampling actions, where  
\begin{equation}
    a_t \sim p_\theta(a_t | o_t, G_t) p_\theta(G_t | o_t) \exp(\kappa G_t - \eta(\kappa))),
\end{equation}
where $\kappa$ controls how strongly we want to tilt the distribution towards high returns, and $\eta(.)$ is a normalizing constant, which is typically ignored.
CtRL-Sim adopts exponential tilting of the predicted return distribution for each agent to finely control agent behaviour. We also explicitly model future sequences of states.

